Lazarus Stars: Numerical investigations of stellar evolution with star-lifting as a life extension strategy

The aging and gradual brightening of the Sun will challenge Earth's habitability in the next few billion years. If life exists elsewhere in the Universe, the aging of its host star similarly poses an existential threat. One solution, which we dub a Lazarus star, is for an advanced civilization to remove (or star-lift) mass from their host star at a rate that offsets the increase in luminosity, keeping the flux on the habitable planet(s) constant and extending the lifetime of their star. While this idea has existed since 1985 when it was first proposed by Criswell, numerical investigations of star-lifting have been lacking. Here, we use the stellar evolution code MESA to find mass vs. age and $\dot{M}$ vs. age relations which would hold the flux on surrounding planets constant. We explore initial mass ranging from $0.2{\rm M}_{\odot}$ to $1.2{\rm M}_{\odot}$. For most stars with a mass initially below about $ 0.4 {\rm M}_{\odot}$, we find that star-lifting increases their main-sequence lifetimes up to $500$ Gyr until they approach the hydrogen burning limit and star-lifting is no longer possible. For more massive stars, star-lifting increase main-sequence lifetimes by 1 Gyr to 100 Gyr, though they still enter the red-giant phase. For example, a Sun-like star has a main-sequence lifetime which can be increased by up to 3 Gyr. This requires a mass-loss rate of about $0.05 {\rm M}_{\mathrm{Ceres}}$ per year. We compare star-lifting to other survival strategies and briefly discuss methods for detecting these engineered stars.

==> notes.tex <==

% \begin{figure}
%  \includegraphics[width=\columnwidth]{gen_vs_mist.pdf}
%  \caption{A comparison of mass {\it vs. } age between the MIST evolutionary tracks and Geneva Isochrones for $[Fe/H] = 0$. Interpolation method used is the same in both sets, fixing $LM^2 = 1$, with data available \href{https://github.com/mscoggs/star_lifting}{here}. MIST tracks cover mass $0.1-300 {\rm M}_{\odot}$ and ages up to$ \sim 10^12$. Isochrones from \citealt{Amard_2019} (Geneva1) cover masses of $0.1-1.2 {\rm M}_{\odot}$. Isochrones from \citealt{Mowlavi_2012} (Genveva2) cover masses of $0.5-3.5 {\rm M}_{\odot}$.}
%  \label{fig:gen_vs_mist}
% \end{figure}
%\appendix
%remove interp techniques unless requested
% \begin{figure}
%  \includegraphics[width=\columnwidth]{mass_vs_age_comp.pdf}
%  \caption{A comparison of mass {\it vs. } age (top) for 4 different interpolation techniques across the MIST evolutionary tracks. Colors indicate $log(F)$ when the star on that track begins start lifting, $A_0$}
%  \label{fig:interp_comp}
% \end{figure}


% \section{Notes}
% \subsection{First order approximation to the required $\dot{M}$}
% In general, for MS stars, 
% \begin{equation}
%     \frac{L}{L_{\odot}} = (\frac{M}{{\rm M}_{\odot}})^a
% \end{equation} 

% For $M \sim {\rm M}_{\odot}$, $a =4$ so the change in luminosity due to a change in mass is given by
% \begin{equation}
%     \frac{dL}{dt}\frac{1}{L_{\odot}} = 4\frac{M^3}{M^4_{\odot}}\dot{M}
% \end{equation} We could get further by setting the change in L due to aging equal to the negative of this, but I'm not sure there is a straightforward $L(t)$ relationship.\\

% A different approach uses 
% \begin{equation*}
%     L = 4\pi\sigma R^2T^4
% \end{equation*} and setting $\frac{dL}{dt} = 0$, we need 
% \begin{equation*}
%  2RT^4 \frac{dR}{dt} = -4R^2T^3\frac{dT}{dt}\\
%     \text{or}\\
%     \frac{dR}{dt} = \frac{2R}{T}\frac{dT}{dt}
% \end{equation*}
% To calculate $\frac{dR}{dt}$, assume we're scraping a tiny fraction of the mass from a thin layer on the surface over a short period, so we can approximate the density as constant in time and radius, $\rho(R,T) = \rho_0$. Then calculating the mass of a thin shell as $M_{shell} = \frac{4}{3}\pi (R^3 - R_0) \rho_0$, 
% \begin{align*}
%     \frac{dM_{shell}}{dt} &= 4\pi R^2 \rho_0 \frac{dR}{dt}\\
%     &= 8\pi \rho_0 \frac{R^3}{T} \frac{dT}{dt}\\
% \end{align*}
% Now we need a way to express $\frac{dT}{dt}$ in terms of $\dot{M}$. Pretending we're at a phase where the sun is beginning to puff up, and pretending $\frac{dT}{dt}$ is linear during this, and pretending the star will lose $2,000 K$ over about a billion years, we get $\frac{dT}{dt} = \frac{-2000K}{3*10^{16}s} \sim -10^{-13} [\frac{K}{s}]$. Although realistically, during the beginning of the swelling phase, this number would be significantly smaller. Pretending this is even remotely accurate, we get a rough first order approximation of 
% \begin{align*}
%     \frac{dM_{shell}}{dt}     &= 8\pi \rho_0 \frac{R^3}{T} \frac{dT}{dt}\\
%     &= 8 \pi 10 \frac{(696.34*10^6)^3}{5778} (-10^{-13})\\
%     &= 1.468*10^{25}(-10^{-13})\\
%     &= -1.468*10^{12}[\frac{kg}{s}]\\
%     &= -1.54*10^{-11}[\frac{{\rm M}_{\odot}}{yr}]\\
% \end{align*} or roughly 1 mount Everest ($1.6* 10^{14} kg$) every 100 seconds.

% \subsection{Misc Considerations}
% \begin{itemize}
%     \item Could this be approached numerically? Does there exist a nice $L$ {\it vs. } $T$ relation as a function of age and initial mass? Could use MESA or MIST tracks (going with MIST tracks)
%     \item Do we eventually hit some instability when we fix L and move off the MS branch? Very few stars between the MS branch and the white dwarf area.
%     \item Changes in tidal effects on earth? Would this still require us to put the earth closer to the sun or would we need to do it so slowly that we can't achieve dL/dt =0?
%     \item Maintaining the strength of the Sun's magnetosphere to protect earth from cosmic radiation?
%     \item Angular momentum considerations
% \end{itemize}

% \subsection{dmdt through MIST}
% See notebook at \href{https://github.com/mscoggs/star_lifting}{star\_lifting}. We get $\dot{M} =3 \times 10^{19}kg$, or roughly $10^{-11} {\rm M}_{\odot}$ per year. For stellar winds, we have $\dot{M} = 10^{-14} {\rm M}_{\odot}$ per year, so stellar lifting would dominate. Surprisingly, this agrees well with our first order approximation.
% \subsection{dmdt {\it vs. } stellar companion formula}
% I've explored Roche overflow a bit but it seems like everything is calculated assuming a less massive body accretion onto a heavy body, which makes sense. I don't think a star-lifter heavier than the sun is reasonable, so I'll consider simple Newtonian gravity and check if lifting with some spherical object of smaller mass is possible.\\

% For a small amount of material of mass dm on the surface of the Sun, and a star-lifter of mass $m$ at distance $a$ from the surface of the sun (distance from the chunk of mass dm), the force of gravity is $F_{\text{net}} = F_{\odot} + F_{lift} = Gdm[-\frac{{\rm M}_{\odot}}{R_{\odot}^2} + \frac{m}{a^2} ]$. To actually get this onto our lifter we'd need $F_{\text{net}} >0$, or
% \begin{align*}
%   \frac{m}{a^2} >  \frac{{\rm M}_{\odot}}{R_{\odot}^2} \leftrightarrow \ \ \ a < \sqrt{\frac{m}{{\rm M}_{\odot}}} R_{\odot}\\
% \end{align*} Assuming something of earth-mass is a reasonable mass for a lifter, we'd need $a < 0.002 R_{\odot} = a_{crit}$. Not sure if this is feasible considering $R_{Earth} = 0.009 R_{\odot}$ so we'd need something much denser than earth in order for the radii of the lifter to be smaller than $a_{crit}$.\\

% I'm wondering if an object of earth-mass near the surface of the Sun can lift the mass quickly enough. For orbital velocity, we have $v_o \sim \sqrt{\frac{GM}{R}}$ and for orbits $v = \frac{2\pi r}{T} = \frac{2\pi (R_{\odot}+a)}{T} \sim \frac{2\pi R_{\odot}}{T}$. Then $T \sim \frac{2\pi R_{\odot}}{v} = \frac{2\pi R_{\odot}^{\frac{3}{2}}} {\sqrt{G{\rm M}_{\odot}}} \sim 1e4 [s]$ or about 3 hours.\\

% The total time $\tau$ it takes the matter to travel from the surface of the sun to our lifter for $a=\frac{a_{crit}}{2}$ with $R_{lift} = \frac{a_{crit}}{4}$ is approximated by constant acceleration using the acceleration when $dm$ is on the surface of the star (which overestimates $\tau$) and pretending the lifter is at a fixed position just above dm (which underestimates $\tau$, I'm hoping these roughly cancel out but not likely). Then $\tau \sim \sqrt{\frac{2d}{a_0}} = \sqrt{\frac{2(\frac{1}{2} - \frac{1}{4})a_{crit}}{\frac{F_0}{dm}}} = \sqrt{\frac{\frac{1}{2}a_{crit}}{G[\frac{m}{a^2} - \frac{{\rm M}_{\odot}}{R_{\odot}^2}]}} = \sqrt{\frac{0.5 * 0.002 R_{\odot}}{G \frac{{\rm M}_{\odot}}{R_{\odot}^2}[\frac{3e-6}{(\frac{1}{2}*0.002)^2}-1]}} = \sqrt{\frac{1e-3}{2}}\frac{R_{\odot}^{\frac{3}{2}}}{\sqrt{G{\rm M}_{\odot}}} \sim 50[s]$. So $\tau << T$, meaning something of earth-mass at a distance of $\frac{a_{crit}}{2}$ from the surface of the Sun could be a viable star-lifter, ignoring engineering and density constraints. For something of that radius, $\rho_{av} = \frac{M_{earth}}{\frac{4}{3}\pi (1e-3 R_{\odot})^3} \sim \frac{6e24}{4e-9*3e26} = 5e6 [kg/m^3] \sim 1e3 \rho_{\text{earth}}$

% A more precise calculation coming soon. Sending this to David to hear thoughts, maybe we should consider other forms of star-lifting (kicking up stellar winds through reflective shielding, 

% \subsection{Related Links}
% \begin{itemize}
%     \item Estimating surface density using\\
%     https://physics.stackexchange.com/questions/201235/density-of-the-sun with $R\sim 0.95$ so $\rho_0 = 10 kg/m^3$
%     \item https://worldbuilding.stackexchange.com/questions/126018/how-do-you-non-catastrophically-reduce-the-mass-of-the-sun-by-half
%     \item Possibly useful for numerical stuff\\
%     https://aas.aanda.org/articles/aas/pdf/2000/12/ds1805.pdf
% \end{itemize}
